A Test Suite for Efficient Robustness Evaluation of Face Recognition Systems

Face recognition is a widely used authentication technology in practice, where robustness is required. It is thus essential to have an efficient and easy-to-use method for evaluating the robustness of (possibly third-party) trained face recognition systems. Existing approaches to evaluating the robustness of face recognition systems are either based on empirical evaluation (e.g., measuring attacking success rate using state-of-the-art attacking methods) or formal analysis (e.g., measuring the Lipschitz constant). While the former demands significant user efforts and expertise, the latter is extremely time-consuming. In pursuit of a comprehensive, efficient, easy-to-use and scalable estimation of the robustness of face recognition systems, we take an old-school alternative approach and introduce RobFace, i.e., evaluation using an optimised test suite. It contains transferable adversarial face images that are designed to comprehensively evaluate a face recognition system's robustness along a variety of dimensions. RobFace is system-agnostic and still consistent with system-specific empirical evaluation or formal analysis. We support this claim through extensive experimental results with various perturbations on multiple face recognition systems. To our knowledge, RobFace is the first system-agnostic robustness estimation test suite.

==> Fig-ablation.tex <==
\pgfplotsset{every tick label/.append style={font=\tiny}}

\begin{figure*}[t]
\centering
\scriptsize
\begin{subfigure}{0.225\textwidth}
\centering
\begin{tikzpicture}

\begin{axis}[
shift,
legend style={at={(1,1)},anchor=north west},
xmin=1, xmax=9,
xtick={1,2,3,4,5,6,7,8,9},xticklabels={I, II, III, IV, V, \underline{VI}, \underline{VII}, \underline{VIII}, IX},
width = \linewidth
]


\addplot+[color=domino,mark=square,]
table[x=system, y= b1mask]
{robustness.dat};

% \addplot+[color=mymagenta,mark=triangle,]
% table[x=system, y= maskb2]
% {robustness.dat};

\addplot+[color=catalina_blue,mark=asterisk,]
table[x=system, y= pmask]
{robustness.dat};

\end{axis}
\end{tikzpicture}
\caption{Face mask ($corr =0.99$)}
%\label{fig:row2}
\end{subfigure}
\begin{subfigure}{0.225\textwidth}
\centering
\begin{tikzpicture}

\begin{axis}[
shift,
legend style={at={(1,1)},anchor=north west},
% title={Temperature dependence of CuSO\(_4\cdot\)5H\(_2\)O solubility},
% % xlabel={Face System},
% % ylabel={Solubility [g per 100 g water]},
xmin=1, xmax=9,
% ymin=0, ymax=120,
xtick={1,2,3,4,5,6,7,8,9},xticklabels={I, II, III, IV, V, VI, \underline{VII}, \underline{VIII}, \underline{IX}},
% ytick={0,20,40,60,80,100},
% legend pos=outer north west,
% ymajorgrids=true,
% grid style=dashed,
% enlargelimits=false,
width = \linewidth
% legend style = {font = \scriptsize}],
]


% \addplot[
%     color=domino,
%     mark=square,
%     ]
%     coordinates {
%     (1,23.1)(2,27.5)(3,32)(4,37.8)(5,44.6)(6,61.8)(7,83.8)(8,114)
%     };
%     \legend{CuSO\(_4\cdot\)5H\(_2\)O}

\addplot+[color=domino,mark=square,]
table[x=system, y= b1glass]
{robustness.dat};

% \addplot+[color=green,mark=^,]
% table[x=system, y= b2l2]
% {robustness.dat};

\addplot+[color=catalina_blue,mark=asterisk,]
table[x=system, y= pglass]
{robustness.dat};

% \addplot+[color=catalina_blue,,mark=*]
%     table[meta=glasses]
%     {robustness.dat};
% \addplot+[
%     only marks,
%     scatter,
%     mark=asterisk*,
%     mark size=2.9pt]
%     table[meta=l2]
%     {robustness.dat};    
\end{axis}
\end{tikzpicture}
\caption{Glasses ($corr = 0.90$)}
\label{fig:corrglass}
\end{subfigure}
\begin{subfigure}{0.225\textwidth}
\centering
\begin{tikzpicture}

\begin{axis}[
shift,
legend style={at={(1,1)},anchor=north west},
xmin=1, xmax=9,
xtick={1,2,3,4,5,6,7,8,9},xticklabels={I, II, III, IV, V, \underline{VI}, VII, \underline{VIII}, \underline{IX}},
width = \linewidth
]


\addplot+[color=domino,mark=square,]
table[x=system, y= b1linf]
{robustness.dat};

\addplot+[color=mymagenta,mark=triangle,]
table[x=system, y= b2linf]
{robustness.dat};

\addplot+[color=catalina_blue,mark=asterisk,]
table[x=system, y= plinf]
{robustness.dat};

\end{axis}
\end{tikzpicture}
\caption{$\ell_\infty$ norm ($corr = 0.92$)}
%\label{fig:row2}
\end{subfigure}
\begin{subfigure}{0.225\textwidth}
\centering
\begin{tikzpicture}

\begin{axis}[
shift,
legend style={at={(1.02,1)},anchor=north west},
xmin=1, xmax=9,
xtick={1,2,3,4,5,6,7,8,9},xticklabels={I, II, III, IV, V, \underline{VI}, \underline{VII}, \underline{VIII}, IX},
width = \linewidth
]

\addplot+[color=domino,mark=square,]
table[x=system, y= b1l2]
{robustness.dat};
\addlegendentry{Reference-1}

\addplot+[color=mymagenta,mark=triangle,]
table[x=system, y= b2l2]
{robustness.dat};
\addlegendentry{Reference-2}

\addplot+[color=catalina_blue,mark=asterisk,]
table[x=system, y= pl2]
{robustness.dat};
\addlegendentry{\textsc{RobFace}}

\end{axis}
\end{tikzpicture}
\caption{$\ell_2$ norm ($corr = 0.97$)}
%\label{fig:row2}
\end{subfigure}\\

\begin{subfigure}{0.225\textwidth}
\centering
\begin{tikzpicture}

\begin{axis}[
shift,
legend style={at={(1,1)},anchor=north west},
xmin=1, xmax=9,
xtick={1,2,3,4,5,6,7,8,9},xticklabels={I, II, \underline{III}, \underline{IV}, V, VI, VII, \underline{VIII}, IX},
width = \linewidth
]


\addplot+[color=domino,mark=square,]
table[x=system, y= b1age]
{robustness.dat};

% \addplot+[color=mymagenta,mark=triangle,]
% table[x=system, y= maskb2]
% {robustness.dat};

\addplot+[color=catalina_blue,mark=asterisk,]
table[x=system, y= page]
{robustness.dat};

\end{axis}
\end{tikzpicture}
\caption{Age shift ($corr =0.99$)}
%\label{fig:row2}
\end{subfigure}
\begin{subfigure}{0.225\textwidth}
\centering
\begin{tikzpicture}

\begin{axis}[
shift,
legend style={at={(1,1)},anchor=north west},
xmin=1, xmax=9,
xtick={1,2,3,4,5,6,7,8,9},xticklabels={\underline{I}, II, \underline{III}, IV, V, VI, \underline{VII}, VIII, IX},
width = \linewidth
]


\addplot+[color=domino,mark=square,]
table[x=system, y= b1pose]
{robustness.dat};

% \addplot+[color=mymagenta,mark=triangle,]
% table[x=system, y= maskb2]
% {robustness.dat};

\addplot+[color=catalina_blue,mark=asterisk,]
table[x=system, y= ppose]
{robustness.dat};

\end{axis}
\end{tikzpicture}
\caption{Pose shift ($corr =0.99$)}
%\label{fig:row2}
\end{subfigure}
\begin{subfigure}{0.225\textwidth}
\centering
\begin{tikzpicture}

\begin{axis}[
shift,
legend style={at={(1,1)},anchor=north west},
xmin=1, xmax=9,
xtick={1,2,3,4,5,6,7,8,9},xticklabels={I, II, \underline{III}, \underline{IV}, V, \underline{VI}, VII, VIII, IX},
width = \linewidth
]


\addplot+[color=domino,mark=square,]
table[x=system, y= b1barrel]
{robustness.dat};

% \addplot+[color=mymagenta,mark=triangle,]
% table[x=system, y= maskb2]
% {robustness.dat};

\addplot+[color=catalina_blue,mark=asterisk,]
table[x=system, y= pbarrel]
{robustness.dat};

\end{axis}
\end{tikzpicture}
\caption{Radial ($corr =0.97$)}
%\label{fig:row2}
\end{subfigure}
\begin{subfigure}{0.225\textwidth}
\centering
\begin{tikzpicture}

\begin{axis}[
shift,
legend style={at={(1,1)},anchor=north west},
xmin=1, xmax=9,
xtick={1,2,3,4,5,6,7,8,9},xticklabels={\underline{I}, II, III, IV, V, VI, \underline{VII}, VIII, \underline{IX}},
width = \linewidth
]


\addplot+[color=domino,mark=square,]
table[x=system, y= b1illum]
{robustness.dat};

% \addplot+[color=mymagenta,mark=triangle,]
% table[x=system, y= maskb2]
% {robustness.dat};

\addplot+[color=catalina_blue,mark=asterisk,]
table[x=system, y= pillum]
{robustness.dat};

\end{axis}
\end{tikzpicture}
\caption{Illumination ($corr = 0.99$)}
%\label{fig:row2}
\end{subfigure}
\vspace{-0.3cm}
\caption{We show that the proposed approach, \textsc{RobFace}, correlates well with the reference robust accuracies, with Pearson correlation ranging from 0.9 to 0.99. A random group of face systems is used for tuning, and the rest are for testing. Indices of the testing systems are underlined. Reference-1 is the robust accuracy by searching adversarial examples via PGD~\cite{madry2017towards}. Reference-2 is CLEVER~\cite{weng2018evaluating}, a theoretical robustness evaluation approach.
}
\label{fig:ablation}
\end{figure*}
% \begin{subfigure}{0.225\textwidth}
% \centering
% \begin{tikzpicture}

% \begin{axis}[
% shift,
% legend style={at={(1,1)},anchor=north west},
% xmin=1, xmax=9,
% xtick={1,2,3,4,5,6,7,8,9},xticklabels={I, II, III, IV, V, VI, VII, VIII, IX},
% width = \linewidth
% ]


% \addplot+[color=domino,mark=square,]
% table[x=system, y= b1rect]
% {robustness.dat};

% % \addplot+[color=mymagenta,mark=triangle,]
% % table[x=system, y= maskb2]
% % {robustness.dat};

% \addplot+[color=catalina_blue,mark=asterisk,]
% table[x=system, y= prect]
% {robustness.dat};

% \end{axis}
% \end{tikzpicture}
% \caption{Rectangle patch ($r=0.68$)}
% %\label{fig:row2}
% \end{subfigure}

